A numerically stable algorithm for integrating Bayesian models using Markov melding

When statistical analyses consider multiple data sources, Markov melding provides a method for combining the source-specific Bayesian models. Markov melding joins together submodels that have a common quantity. One challenge is that the prior for this quantity can be implicit, and its prior density must be estimated. We show that error in this density estimate makes the two-stage Markov chain Monte Carlo sampler employed by Markov melding unstable and unreliable. We propose a robust two-stage algorithm that estimates the required prior marginal self-density ratios using weighted samples, dramatically improving accuracy in the tails of the distribution. The stabilised version of the algorithm is pragmatic and provides reliable inference. We demonstrate our approach using an evidence synthesis for inferring HIV prevalence, and an evidence synthesis of A/H1N1 influenza.

==> tex-input/kde-calcs/indefinite-integral-0030.tex <==
\begin{align}
  \kappa &\approx 
  \int_{\mathcal{R}}
    \frac{1} {\text{K}}
    \hat{\pd}(\phi) \w(\phi;\xi) 
  \text{d}\phi \nonumber \\ 
  &=
  \frac {
    \frac{1}{\Nx} \sum\limits_{\sampleindex = 1}^{\Nx}
      S(\phi_\sampleindex, h^2, \mu, \sigma^2)
      \left(
        \Phi(b; \mu_{p, \sampleindex}, \sigma^2_{p}) - \Phi(a; \mu_{p, \sampleindex}, \sigma^2_{p})
      \right)    
  } {
    \frac{1}{\Nx} \sum\limits_{\sampleindex = 1}^{\Nx}
      S(\phi_\sampleindex, h^2, \mu, \sigma^2)
  }
  \label{eqn:final_res}
\end{align}

==> tex-input/kde-calcs/maths-setup-0020.tex <==
\begin{equation}
  \int_{\mathcal{R}} \frac{1}{Z_{2}} \pd(\phi) \w(\phi;\xi) \text{d}\phi 
  =
  \kappa,
  \label{eqn:target_equality}
\end{equation}

==> tex-input/kde-calcs/normalising-constant-0020.tex <==
\begin{equation*}
  \begin{gathered}
  S(\phi_\sampleindex, h^2, \mu, \sigma^2) = \frac{
    1
  } {
    \sqrt{2 \pi (h^2 + \sigma^2)}
  }
  \text{exp} \left\{
    -\frac{
       (\phi_{\sampleindex} - \mu)^2
    } {
      2(h^2 + \sigma^2)
    }
  \right\},
  \\
  \mu_{p, \sampleindex} = \frac{
    h^2 \mu + \sigma^2 \phi_{\sampleindex}
  } {
    h^2 + \sigma^2
  }, \quad
  \sigma^2_{p} = \frac{
    h^2 \sigma^2
  } {
    h^2 + \sigma^2
  }.
  \end{gathered}
  \label{eqn:s-norm-const-def}
\end{equation*}

==> tex-input/kde-calcs/product-gaussians-0010.tex <==
\begin{align}
  \text{K}_{h}&(\phi - \phi_{\sampleindex}) \w(\phi;\xi) = \nonumber \\
    & \frac{
      S(\phi_\sampleindex, h^2, \mu, \sigma^2)
    } {
      \sqrt{2 \pi \sigma^2_{p}}
    }
    \text{exp} \left\{
      - \frac{
        (\phi - \mu_{p, \sampleindex})^{2}
      } {
        2 \sigma^2_{p} 
      }
    \right\}
  \label{eqn:product-gaussians}
\end{align}

==> tex-input/markov-melding/0081-melded-joint-two-hiv.tex <==
\begin{equation*}
  \pd_{\text{meld}}(\phi, \psi_{1}, \psi_{2} \mid Y_{1}, Y_{2}) \, \propto \,
  \ppoolphi
  \frac{\pd_{1}(\phi, \psi_{1}, Y_{1})}{\pd_{1}(\phi)}
  \frac{\pd_{2} (\phi, \psi_{2}, Y_{2})}{\pd_{2}(\phi)}.
  \label{eqn:melded-joint-two-hiv}
\end{equation*}

==> tex-input/pre.tex <==
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{url}

% I always seem to need tikz for something
\usepackage{tikz}
\usetikzlibrary{positioning, shapes, intersections, through, backgrounds, fit, decorations.pathmorphing}

\usepackage{setspace}
\onehalfspacing

\usepackage{lineno}
% \linenumbers

% required for landscape pages. beware, they back the build very slow.
\usepackage{pdflscape}

% table
\usepackage{longtable}
\usepackage{booktabs}
\usepackage{caption}

\usepackage{accents}


% \usepackage[colorlinks=true, urlcolor=citecolor, linkcolor=citecolor, citecolor=citecolor]{hyperref}


% cross out math
\usepackage[makeroom]{cancel}

\setcounter{secnumdepth}{3}

% pd stands for: probability distribution and is useful to distringuish
% marignals for probabilities specifically p(p_{1}) and the like.
\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\widehat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \widehat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\widehat{#1}}}}

\newcommand{\pd}{\text{p}}
\newcommand{\q}{\text{q}}
\newcommand{\w}{\text{w}}
\newcommand{\pdr}{\text{r}}
\newcommand{\pdrh}{\widehat{\text{r}}}

% melding
\newcommand{\ppoolphi}{\pd_{\text{pool}}(\phi)}
\newcommand{\s}{\text{s}}
\newcommand{\tofs}{\text{t}}
\newcommand{\m}{\text{m}}
\newcommand{\uofp}{\text{u}}
% direct density estimate - replaces lambda.
\newcommand{\ddest}{\text{s}}

% constants - usually sizes of things
\newcommand{\Nx}{N}
\newcommand{\Nnu}{\text{N}_{\text{nu}}}
\newcommand{\Nde}{\text{N}_{\text{de}}}
\newcommand{\Nmc}{\text{N}_{\text{mc}}}
\newcommand{\Nw}{W}
\newcommand{\Nm}{M}

% locales - could switch to x and x'
\newcommand{\xnu}{x_{\text{nu}}}
\newcommand{\xde}{x_{\text{de}}}
\newcommand{\phinu}{\phi_{\text{nu}}}
\newcommand{\phide}{\phi_{\text{de}}}

% sugiyama stuff
\newcommand{\pdnu}{\pd_{\text{nu}}}
\newcommand{\pdde}{\pd_{\text{de}}}

% indices 
\newcommand{\wfindex}{w}
\newcommand{\sampleindex}{n}
\newcommand{\modelindex}{m}



==> tex-input/wsre/0012-example-wf.tex <==
\begin{equation*}
  \w(\phi;\xi) = 
    \frac{1} {\sqrt{2 \pi \sigma^{2}}}
    \text{exp} \left\{
      - \frac{1}{2 \sigma^{2}}
      (\phi - \mu)^2
    \right\},
    \quad
    \xi = (\mu, \sigma^{2}),
  \label{eqn:example-wf}
\end{equation*}

==> tex-input/wsre/0041-joint-ddest.tex <==
\begin{equation}
  \hat{\ddest}_{\wfindex} (\xnu, \xde) = 
    \hat{\ddest}_{\wfindex} (\xnu)
    \hat{\ddest}_{\wfindex} (\xde).
  \label{eqn:joint-ddest}
\end{equation}
